Bootstrapping a User-Centered Task-Oriented Dialogue System

We present TacoBot, a task-oriented dialogue system built for the inaugural Alexa Prize TaskBot Challenge, which assists users in completing multi-step cooking and home improvement tasks. TacoBot is designed with a user-centered principle and aspires to deliver a collaborative and accessible dialogue experience. Towards that end, it is equipped with accurate language understanding, flexible dialogue management, and engaging response generation. Furthermore, TacoBot is backed by a strong search engine and an automated end-to-end test suite. In bootstrapping the development of TacoBot, we explore a series of data augmentation strategies to train advanced neural language processing models and continuously improve the dialogue experience with collected real conversations. At the end of the semifinals, TacoBot achieved an average rating of 3.55/5.0.

==> intro-v1.tex <==
\pdfoutput=1
\section{Introduction}
%\rc{Ready for revision}
\nop{
Background: TODO next version
Building a task-oriented dialogue system has long been an open challenge \citep{BOBROW1977155}. Although pre-trained language models have lifted the state-of-the-art performance in automatic benchmarks \citep{ham-etal-2020-end, wu-etal-2020-tod}, fine-tuning them with large-scale data is still crucial to yield satisfying results, not to mention the noisy and long-tailed distribution in real world dialogue data. 
}

%\rc{Aim} 
In this paper, we present \taskbot, a dialogue system built for the first Alexa Prize TaskBot Challenge, which assists users in completing multi-step cooking and home improvement tasks. Unlike static benchmarks \citep{budzianowski-etal-2018-multiwoz, Rastogi_Zang_Sunkara_Gupta_Khaitan_2020}, Alexa Prize keeps attracting new users to interact and evaluate our system, enabling us to collect realistic conversation data and develop a satisfying product. This dynamic influx of users also motivates us to build a user-centered dialogue system that aspires to deliver a collaborative and accessible conversation experience. To this end, TacoBot must demonstrate many capabilities, including accurate language understanding, flexible dialogue management, and engaging response generation. 

%\rc{Challenge}
These needs pose several challenges to building a TaskBot from scratch: (1) \textit{data insufficiency} because neural models are data-hungry and crowdsourcing sufficient training data can be costly, (2) \textit{domain adaptation} for specific language usage in cooking and home improvement instructions, and (3) \textit{user noise} that increases model prediction difficulty for irregular input patterns. To conquer these challenges, we adopt three strategies to bootstrap the development process of TacoBot.

%\rc{Methods} 
First, we extract few-shot examples from collected conversations to synthesize large-scale training data. Leveraging GPT-3, a large pre-trained language model, we build several accurate language understanding models, which set a reliable foundation for our system. Second, we annotate the conversations to build suitable evaluation datasets for most system components. Compared to simulated data, these datasets better reflect the authentic distribution of user inputs and reveals fatal deficiencies of our models. Finally, we turn observed user behaviors into meaningful design guidelines. With a clear direction, we continuously improve the flexibility of our dialogue management module and the engagingness of our response generation templates. 

%\rc{Results} 
Further backed by a strong search engine and a comprehensive end-to-end test suite, TacoBot has achieved an average rating of $3.49/5.0$ in the semifinals. ...
\rc{As of 3/23, update this Friday}
